Extensive Online Shock Model Database

We present a new database of fully radiative shock models calculated with the shock and photoionization code MAPPINGS V. The database architecture is built to contain diverse shock grids comprising of multiple shock parameters. It can be easily accessible through the MySQL protocol. Intensities of spectral lines from infrared to X-rays are stored along with other useful outputs such as the ionic fractions/temperature, integrated densities, etc. A web page was created in other to explore interactively the database as it evolves with time. Examples of its usage is given using the Python language.

==> tables/abundancesGutkin.tex <==
\begin{table}[ht]
\scriptsize
\caption{Interstellar abundances of the 30 lightest chemical elements for Z$_{ISM}$ = Z$_\odot$ = 0.01524.}
\label{tab:abundTableGutkin}
\begin{center}
\begin{tabular}{lccccc}
\hline
Element & log($n_{i}$/$n_{H}$) \\
\hline
H  &  0.00  \\
He & -1.01  \\
Li & -10.99 \\
Be & -10.63 \\
B  & -9.47 \\
C  & -3.53 \\
N  & -4.32 \\
O  & -3.17 \\
F  & -7.47 \\
Ne & -4.01 \\
Na & -5.70 \\
Mg & -4.45 \\
Al & -5.56 \\
Si & -4.48 \\
P  & -6.57 \\
S  & -4.87 \\
Cl & -6.53 \\
Ar & -5.63 \\
K  & -6.92 \\
Ca & -5.67 \\
Sc & -8.86 \\
Ti & -7.01 \\
V  & -8.03 \\
Cr & -6.36 \\
Mn & -6.64 \\
Fe & -4.51 \\
Co & -7.11 \\ 
Ni & -5.78 \\
Cu & -7.82 \\
Zn & -7.43 \\
\hline
\end{tabular}
\end{center}
\end{table}

==> tables/abundancesList.tex <==
\begin{table*}[ht]
\small
\caption{Abundances sets \Lchg{used in} the database}
\label{tab:abundancesTable}
\begin{center}
\begin{tabular}{ccccc}
\hline
Element & ID-1 & ID-2 & ID-3 \\
\hline
He & -1.09  & -1.01  & -1.05  &\\
Li & -      & -      & -      &\\
Be & -      & -      & -      &\\
B  & -      & -      & -      &\\
C  & -4.24  & -3.44  & -3.96  &\\
N  & -5.37  & -3.95  & -4.86  &\\
O  & -3.97  & -3.07  & -3.65  &\\
F  & -      & -      & - 	  &\\
Ne & -4.73  & -3.91  & -4.39  &\\
Na & -5.92  & -      & -4.85  &\\
Mg & -5.01  & -4.42  & -4.53  &\\
Al & -5.60  & -5.53  & -4.28  &\\
Si & -4.69  & -4.45  & -5.29  &\\
P  & -      & -      & -      &\\
S  & -5.41  & -4.79  & -7.23  &\\
Cl & -7.30  & -      & -      &\\
Ar & -6.29  & -5.44  & -5.71  &\\
K  & -      & -      & -      &\\
Ca & -6.16  & -5.88  & -6.03  &\\
Sc & -      & -      & -      &\\
Ti & -      & -      & -      &\\
V  & -      & -      & -      &\\
Cr & -      & -      & -      &\\
Mn & -      & -      & -      &\\
Fe & -5.11  & -4.63  & -4.77  &\\
Co & -      & -      & -      &\\
Ni & -6.14  & -      & -6.04  &\\
Cu & -      & -      & -      &\\
Zn & -      & -      & -      &\\
\hline
X  & 0.7535 & 0.7073 & 0.7334 &\\
Y  & 0.2432 & 0.2745 & 0.2596 &\\
Z  & 0.0033 & 0.0183 & 0.0070 &\\
\hline
\end{tabular}
\end{center}
\end{table*}
